$\text{DC}^2$: Dual-Camera Defocus Control by Learning to Refocus

Smartphone cameras today are increasingly approaching the versatility and quality of professional cameras through a combination of hardware and software advancements. However, fixed aperture remains a key limitation, preventing users from controlling the depth of field (DoF) of captured images. At the same time, many smartphones now have multiple cameras with different fixed apertures -- specifically, an ultra-wide camera with wider field of view and deeper DoF and a higher resolution primary camera with shallower DoF. In this work, we propose $\text{DC}^2$, a system for defocus control for synthetically varying camera aperture, focus distance and arbitrary defocus effects by fusing information from such a dual-camera system. Our key insight is to leverage real-world smartphone camera dataset by using image refocus as a proxy task for learning to control defocus. Quantitative and qualitative evaluations on real-world data demonstrate our system's efficacy where we outperform state-of-the-art on defocus deblurring, bokeh rendering, and image refocus. Finally, we demonstrate creative post-capture defocus control enabled by our method, including tilt-shift and content-based defocus effects.

==> figures_tex/rebuttal_uw.tex <==
\begin{figure}[h!]
    \centering
    \mfigure{0.45}{match_fov_uw_final_book_modified.png}
    \mfigure{0.45}{match_fov_uw_final_kitchen_modified.png}
    
    \mfigure{0.45}{match_fov_uw_final_micro_modified.png}
    \mfigure{0.45}{match_fov_uw_final_cafeteria_modified.png}

    \caption{UW inputs. UW images have a deeper DoF and are almost all-in-focus (zoom in for details).}
    \label{fig:rebuttal_uw}
\end{figure}

